Everest: GPU-Accelerated System For Mining Temporal Motifs

Temporal motif mining is the task of finding the occurrences of subgraph patterns within a large input temporal graph that obey the specified structural and temporal constraints. Despite its utility in several critical application domains that demand high performance (e.g., detecting fraud in financial transaction graphs), the performance of existing software is limited on commercial hardware platforms, in that it runs for tens of hours. This paper presents Everest - a system that efficiently maps the workload of mining (supports both enumeration and counting) temporal motifs to the highly parallel GPU architecture. In particular, using an input temporal graph and a more expressive user-defined temporal motif query definition compared to prior works, Everest generates an execution plan and runtime primitives that optimize the workload execution by exploiting the high compute throughput of a GPU. Everest generates motif-specific mining code to reduce long-latency memory accesses and frequent thread divergence operations. Everest incorporates novel low-cost runtime mechanisms to enable load balancing to improve GPU hardware utilization. To support large graphs that do not fit on GPU memory, Everest also supports multi-GPU execution by intelligently partitioning the edge list that prevents inter-GPU communication. Everest hides the implementation complexity of presented optimizations away from the targeted system user for better usability. Our evaluation shows that, using proposed optimizations, Everest improves the performance of a baseline GPU implementation by 19x, on average.

==> tmp/backup-vldb-bib <==
@article{barabasi2013network,
  title={Network science},
  author={Barab{\'a}si, Albert-L{\'a}szl{\'o}},
  journal={Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
  volume={371},
  number={1987},
  pages={20120375},
  year={2013},
  publisher={The Royal Society Publishing}
}

@book{lewis2011network,
  title={Network science: Theory and applications},
  author={Lewis, Ted G},
  year={2011},
  publisher={John Wiley \& Sons}
}

@inproceedings{diff_dynamic_temporal, 
author = {Rozenshtein, Polina and Gionis, Aristides}, 
title = {Mining Temporal Networks}, 
year = {2019},
booktitle = {Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining}, pages = {3225–3226}, numpages = {2}, keywords = {temporal networks, graph mining, data mining}, 
}

@misc{motifs_wiki,
    author = "{Wikipedia contributors}",
    title = "Network motif --- {Wikipedia}{,} The Free Encyclopedia",
    year = "2022",
    url = "https://en.wikipedia.org/w/index.php?title=Network_motif&oldid=1077144331",
    note = "[Online; accessed 20-April-2022]"
  }
  
  @inproceedings{hajdu2020temporal,
  title={Temporal network analytics for fraud detection in the banking sector},
  author={Hajdu, L{\'a}szl{\'o} and Kr{\'e}sz, Mikl{\'o}s},
  booktitle={ADBIS, TPDL and EDA 2020 Common Workshops and Doctoral Consortium},
  pages={145--157},
  year={2020},
  organization={Springer}
}

  @article{milo2002network,
  title={Network motifs: simple building blocks of complex networks},
  author={Milo, Ron and Shen-Orr, Shai and Itzkovitz, Shalev and Kashtan, Nadav and Chklovskii, Dmitri and Alon, Uri},
  journal={Science},
  volume={298},
  number={5594},
  pages={824--827},
  year={2002},
  publisher={American Association for the Advancement of Science}
}

@article{tu2018network,
  title={Network classification in temporal networks using motifs},
  author={Tu, Kun and Li, Jian and Towsley, Don and Braines, Dave and Turner, Liam D},
  journal={arXiv preprint arXiv:1807.03733},
  year={2018}
}

  @article{newman2003structure,
  title={The structure and function of complex networks},
  author={Newman, Mark EJ},
  journal={SIAM review},
  volume={45},
  number={2},
  pages={167--256},
  year={2003},
  publisher={SIAM}
}
 
 @article{alon2007network,
  title={Network motifs: theory and experimental approaches},
  author={Alon, Uri},
  journal={Nature Reviews Genetics},
  volume={8},
  number={6},
  pages={450--461},
  year={2007},
  publisher={Nature Publishing Group}
}

@article{holme2012temporal,
  title={Temporal networks},
  author={Holme, Petter and Saram{\"a}ki, Jari},
  journal={Physics reports},
  volume={519},
  number={3},
  pages={97--125},
  year={2012},
  publisher={Elsevier}
}

@article{shen2002network,
  title={Network motifs in the transcriptional regulation network of Escherichia coli},
  author={Shen-Orr, Shai S and Milo, Ron and Mangan, Shmoolik and Alon, Uri},
  journal={Nature genetics},
  volume={31},
  number={1},
  pages={64--68},
  year={2002},
  publisher={Nature Publishing Group}
}

% first appearance of temporal motifs
@article{rocha2011simulated,
  title={Simulated epidemics in an empirical spatiotemporal network of 50,185 sexual contacts},
  author={Rocha, Luis EC and Liljeros, Fredrik and Holme, Petter},
  journal={PLoS computational biology},
  volume={7},
  number={3},
  pages={e1001109},
  year={2011},
  publisher={Public Library of Science San Francisco, USA}
}

@article{lee2012exploiting,
  title={Exploiting temporal network structures of human interaction to effectively immunize populations},
  author={Lee, Sungmin and Rocha, Luis EC and Liljeros, Fredrik and Holme, Petter},
  journal={PloS one},
  volume={7},
  number={5},
  pages={e36439},
  year={2012},
  publisher={Public Library of Science San Francisco, USA}
}

@article{kovanen2011temporal,
  title={Temporal motifs in time-dependent networks},
  author={Kovanen, Lauri and Karsai, M{\'a}rton and Kaski, Kimmo and Kert{\'e}sz, J{\'a}nos and Saram{\"a}ki, Jari},
  journal={Journal of Statistical Mechanics: Theory and Experiment},
  volume={2011},
  number={11},
  pages={P11005},
  year={2011},
  publisher={IOP Publishing}
}

% Temporal motifs applications
@inproceedings{huang2014mining,
  title={Mining triadic closure patterns in social networks},
  author={Huang, Hong and Tang, Jie and Wu, Sen and Liu, Lu and Fu, Xiaoming},
  booktitle={Proceedings of the 23rd international conference on World wide web},
  pages={499--504},
  year={2014}
}

@INPROCEEDINGS{lahiri2007structure,
  author={Lahiri, Mayank and Berger-Wolf, Tanya Y.},
  booktitle={2007 IEEE Symposium on Computational Intelligence and Data Mining}, 
  title={Structure Prediction in Temporal Networks using Frequent Subgraphs}, 
  year={2007},
  volume={},
  number={},
  pages={35-42},
  doi={10.1109/CIDM.2007.368850}}


@article{hulovatyy2015exploring,
  title={Exploring the structure and function of temporal networks with dynamic graphlets},
  author={Hulovatyy, Yuriy and Chen, Huili and Milenkovi{\'c}, Tijana},
  journal={Bioinformatics},
  volume={31},
  number={12},
  pages={i171--i180},
  year={2015},
  publisher={Oxford University Press}
}

@article{kondor2014inferring,
  title={Inferring the interplay between network structure and market effects in Bitcoin},
  author={Kondor, D{\'a}niel and Csabai, Istv{\'a}n and Sz{\"u}le, J{\'a}nos and P{\'o}sfai, M{\'a}rton and Vattay, G{\'a}bor},
  journal={New Journal of Physics},
  volume={16},
  number={12},
  pages={125003},
  year={2014},
  publisher={IOP Publishing}
}

@article{kovanen2013temporal,
  title={Temporal motifs reveal homophily, gender-specific patterns, and group talk in call sequences},
  author={Kovanen, Lauri and Kaski, Kimmo and Kert{\'e}sz, J{\'a}nos and Saram{\"a}ki, Jari},
  journal={Proceedings of the National Academy of Sciences},
  volume={110},
  number={45},
  pages={18070--18075},
  year={2013},
  publisher={National Acad Sciences}
}

@inproceedings{shao2013temporal,
  title={A temporal motif mining approach to unsupervised energy disaggregation: Applications to residential and commercial buildings},
  author={Shao, Huijuan and Marwah, Manish and Ramakrishnan, Naren},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={27},
  number={1},
  pages={1327--1333},
  year={2013}
}

@inproceedings{meydan2013prediction,
  title={Prediction of peptides binding to MHC class I and II alleles by temporal motif mining},
  author={Meydan, Cem and Otu, Hasan H and Sezerman, Osman U{\u{g}}ur},
  booktitle={BMC bioinformatics},
  volume={14},
  number={2},
  pages={1--11},
  year={2013},
  organization={Springer}
}

@article{bouritsas2022improving,
  title={Improving graph neural network expressivity via subgraph isomorphism counting},
  author={Bouritsas, Giorgos and Frasca, Fabrizio and Zafeiriou, Stefanos P and Bronstein, Michael},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2022},
  publisher={IEEE}
}

@article{rossi2020temporal,
  title={Temporal graph networks for deep learning on dynamic graphs},
  author={Rossi, Emanuele and Chamberlain, Ben and Frasca, Fabrizio and Eynard, Davide and Monti, Federico and Bronstein, Michael},
  journal={arXiv preprint arXiv:2006.10637},
  year={2020}
}

@inproceedings{glasser2013bridging,
  title={Bridging the gap: A pragmatic approach to generating insider threat data},
  author={Glasser, Joshua and Lindauer, Brian},
  booktitle={2013 IEEE Security and Privacy Workshops},
  pages={98--104},
  year={2013},
  organization={IEEE}
}

% algorithmic complexity

@inproceedings{cook1971complexity,
  title={The complexity of theorem-proving procedures},
  author={Cook, Stephen A},
  booktitle={Proceedings of the third annual ACM symposium on Theory of computing},
  pages={151--158},
  year={1971}
}

@article{pan2011path,
  title={Path lengths, correlations, and centrality in temporal networks},
  author={Pan, Raj Kumar and Saram{\"a}ki, Jari},
  journal={Physical Review E},
  volume={84},
  number={1},
  pages={016105},
  year={2011},
  publisher={APS}
}


@inproceedings{paranjape2017motifs,
  title={Motifs in temporal networks},
  author={Paranjape, Ashwin and Benson, Austin R and Leskovec, Jure},
  booktitle={Proceedings of the tenth ACM international conference on web search and data mining},
  pages={601--610},
  year={2017}
}

@inproceedings{mackey2018chronological,
  title={A chronological edge-driven approach to temporal subgraph isomorphism},
  author={Mackey, Patrick and Porterfield, Katherine and Fitzhenry, Erin and Choudhury, Sutanay and Chin, George},
  booktitle={2018 IEEE international conference on big data (big data)},
  pages={3972--3979},
  year={2018},
  organization={IEEE}
}

@inbook{graphpi, author = {Shi, T. and Zhai, M. and Xu, Y. and Zhai, J.}, title = {GraphPi: High Performance Graph Pattern Matching through Effective Redundancy Elimination}, year = {2020}, isbn = {9781728199986}, publisher = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis}, abstract = {Graph pattern matching, which aims to discover structural patterns in graphs, is considered one of the most fundamental graph mining problems in many real applications. Despite previous efforts, existing systems face two main challenges. First, inherent symmetry existing in patterns can introduce a large amount of redundant computation. Second, different matching orders for a pattern have significant performance differences and are quite hard to predict. When these factors are mixed, this problem becomes extremely complicated. High efficient pattern matching remains an open problem currently.To address these challenges, we propose GraphPi, a high performance distributed pattern matching system. GraphPi utilizes a new algorithm based on 2-cycles in group theory to generate multiple sets of asymmetric restrictions, where each set can eliminate redundant computation completely. We further design an accurate performance model to determine the optimal matching order and asymmetric restriction set for efficient pattern matching. We evaluate GraphPi on Tianhe-2A supercomputer. Results show that GraphPi outperforms the state-of-the-art system, by up to 105\texttimes{} for 6 real-world graph datasets on a single node. We also scale GraphPi to 1,024 computing nodes (24,576 cores).}, booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis}, articleno = {100}, numpages = {14} }

@inproceedings{mawhirter2019automine,
  title={Automine: harmonizing high-level abstraction and high performance for graph mining},
  author={Mawhirter, Daniel and Wu, Bo},
  booktitle={Proceedings of the 27th ACM Symposium on Operating Systems Principles},
  pages={509--523},
  year={2019}
}

@article{mawhirter2019graphzero,
  title={Graphzero: Breaking symmetry for efficient graph mining},
  author={Mawhirter, Daniel and Reinehr, Sam and Holmes, Connor and Liu, Tongping and Wu, Bo},
  journal={arXiv preprint arXiv:1911.12877},
  year={2019}
}

@inproceedings{wang2020efficient,
  title={Efficient sampling algorithms for approximate temporal motif counting},
  author={Wang, Jingjing and Wang, Yanhao and Jiang, Wenjun and Li, Yuchen and Tan, Kian-Lee},
  booktitle={Proceedings of the 29th ACM international conference on information \& knowledge management},
  pages={1505--1514},
  year={2020}
}

@article{kumar20182scent,
  title={2scent: An efficient algorithm to enumerate all simple temporal cycles},
  author={Kumar, Rohit and Calders, Toon},
  journal={Proceedings of the VLDB Endowment},
  volume={11},
  number={11},
  pages={1441--1453},
  year={2018}
}

@article{liu2018sampling,
  title={A sampling framework for counting temporal motifs},
  author={Liu, Paul and Benson, Austin and Charikar, Moses},
  journal={arXiv preprint arXiv:1810.00980},
  year={2018}
}

@inproceedings{sarpe2021presto,
  title={PRESTO: Simple and Scalable Sampling Techniques for the Rigorous Approximation of Temporal Motif Counts},
  author={Sarpe, Ilie and Vandin, Fabio},
  booktitle={Proceedings of the 2021 SIAM International Conference on Data Mining (SDM)},
  pages={145--153},
  year={2021},
  organization={SIAM}
}

@inproceedings{talati2021deep,
  title={A Deep Dive Into Understanding The Random Walk-Based Temporal Graph Learning},
  author={Talati, Nishil and Jin, Di and Ye, Haojie and Brahmakshatriya, Ajay and Dasika, Ganesh and Amarasinghe, Saman and Mudge, Trevor and Koutra, Danai and Dreslinski, Ronald},
  booktitle={2021 IEEE International Symposium on Workload Characterization (IISWC)},
  pages={87--100},
  year={2021},
  organization={IEEE}
}

@INPROCEEDINGS{flexminer,
  author={X. Chen and T. Huang and S. Xu and T. Bourgeat and C. Chung and Arvind},
  booktitle={Proceedings of the ACM/IEEE 47th Annual International Symposium on Computer Architecture},
  title={FlexMiner: A Pattern-Aware Accelerator for Graph Pattern Mining}, 
  year={2021},
  volume={},
  number={},
  pages={581-594}}
  
  @INPROCEEDINGS{gramer,
  author={Yao, P. and Zheng, L. and Zeng, Z. and Huang, Y. and Gui, C. and Liao, X. and Jin, H. and Xue, J.},
  booktitle={2020 53rd Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)}, 
  title={A Locality-Aware Energy-Efficient Accelerator for Graph Mining Applications}, 
  year={2020},
  volume={},
  number={},
  pages={895-907},
  doi={10.1109/MICRO50266.2020.00077}}
  
  @inproceedings{sparsecore, author = {Rao, Gengyu and Chen, Jingji and Yik, Jason and Qian, Xuehai}, title = {SparseCore: Stream ISA and Processor Specialization for Sparse Computation}, year = {2022}, isbn = {9781450392051}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/3503222.3507705}, doi = {10.1145/3503222.3507705}, abstract = {Computation on sparse data is becoming increasingly important for many applications. Recent sparse computation accelerators are designed for specific algorithm/application, making them inflexible with software optimizations. This paper proposes SparseCore, the first general-purpose processor extension for sparse computation that can flexibly accelerate complex code patterns and fast-evolving algorithms. We extend the instruction set architecture (ISA) to make stream or sparse vector first-class citizens, and develop efficient architectural components to support the stream ISA. The novel ISA extension intrinsically operates on streams, realizing both efficient data movement and computation. The simulation results show that SparseCore achieves significant speedups for sparse tensor computation and graph pattern computation.}, booktitle = {Proceedings of the 27th ACM International Conference on Architectural Support for Programming Languages and Operating Systems}, pages = {186–199}, numpages = {14}, keywords = {Graph analytics, Deep learning, Stream ISA, Sparse computation acceleration}, location = {Lausanne, Switzerland}, series = {ASPLOS 2022} }


@inbook{fingers, author = {Chen, Qihang and Tian, Boyu and Gao, Mingyu}, title = {FINGERS: Exploiting Fine-Grained Parallelism in Graph Mining Accelerators}, year = {2022}, isbn = {9781450392051}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/3503222.3507730}, abstract = {Graph mining is an emerging application of high importance and also with high complexity, thus requiring efficient hardware acceleration. Current accelerator designs only utilize coarse-grained parallelism, leaving large room for further optimizations. Our key insight is to fully exploit fine-grained parallelism to overcome the existing issues of hardware underutilization, inefficient resource provision, and limited single-thread performance under imbalanced loads. Targeting pattern-aware graph mining algorithms, we first comprehensively identify and analyze the abundant fine-grained parallelism at the branch, set, and segment levels during search tree exploration and set operations. We then propose a novel graph mining accelerator, FINGERS, which effectively exploits these multiple levels of fine-grained parallelism to achieve significant performance improvements. FINGERS mainly enhances the design of each single processing element with parallel compute units for set operations, and efficient techniques for task scheduling, load balancing, and data aggregation. FINGERS outperforms the state-of-the-art design by 2.8\texttimes{} on average and up to 8.9\texttimes{} with the same chip area. We also demonstrate that different patterns and different graphs exhibit drastically different parallelism opportunities, justifying the necessity of exploiting all levels of fine-grained parallelism in FINGERS.}, booktitle = {Proceedings of the 27th ACM International Conference on Architectural Support for Programming Languages and Operating Systems}, pages = {43–55}, numpages = {13} }

@INPROCEEDINGS{ndminer,
  author={Talati, Nishil and Ye, Haojie and Yang, Yichen and  Belayneh, Leul and Chen, Kuan-Yu and Blaauw, David and Mudge, Trevor and Dreslinski, Ronald},
  booktitle={Proceedings of the ACM/IEEE 48th Annual International Symposium on Computer Architecture},
  title={NDMiner: Accelerating Graph Pattern Mining Using Near Data Processing}, 
  year={2022}}
  
  @INPROCEEDINGS{graph_accelerator1,  author={Ham, Tae Jun and Wu, Lisa and Sundaram, Narayanan and Satish, Nadathur and Martonosi, Margaret},  booktitle={2016 49th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},   title={Graphicionado: A high-performance and energy-efficient accelerator for graph analytics},   year={2016},  volume={},  number={},  pages={1-13},  doi={10.1109/MICRO.2016.7783759}}
  
  @INPROCEEDINGS{7284059,  author={Ahn, Junwhan and Hong, Sungpack and Yoo, Sungjoo and Mutlu, Onur and Choi, Kiyoung},  booktitle={2015 ACM/IEEE 42nd Annual International Symposium on Computer Architecture (ISCA)},   title={A scalable processing-in-memory accelerator for parallel graph processing},   year={2015},  volume={},  number={},  pages={105-117},  doi={10.1145/2749469.2750386}}
  
  @INPROCEEDINGS{dom7,  author={Mukkara, Anurag and Beckmann, Nathan and Abeydeera, Maleen and Ma, Xiaosong and Sanchez, Daniel},  booktitle={2018 51st Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},   title={Exploiting Locality in Graph Analytics through Hardware-Accelerated Traversal Scheduling},   year={2018},  volume={},  number={},  pages={1-14},  doi={10.1109/MICRO.2018.00010}}
  
  @INPROCEEDINGS{dom8,
  author={Song, Linghao and Zhuo, Youwei and Qian, Xuehai and Li, Hai and Chen, Yiran},
  booktitle={2018 IEEE International Symposium on High Performance Computer Architecture (HPCA)}, 
  title={GraphR: Accelerating Graph Processing Using ReRAM}, 
  year={2018},
  volume={},
  number={},
  pages={531-543},
  doi={10.1109/HPCA.2018.00052}}
  
  @INPROCEEDINGS{dom11,  author={Addisie, Abraham and Kassa, Hiwot and Matthews, Opeoluwa and Bertacco, Valeria},  booktitle={2018 IEEE International Symposium on Workload Characterization (IISWC)},   title={Heterogeneous Memory Subsystem for Natural Graph Analytics},   year={2018},  volume={},  number={},  pages={134-145},  doi={10.1109/IISWC.2018.8573480}}
  


@INPROCEEDINGS{dom1,  author={Ozdal, Muhammet Mustafa and Yesil, Serif and Kim, Taemin and Ayupov, Andrey and Greth, John and Burns, Steven and Ozturk, Ozcan},  booktitle={2016 ACM/IEEE 43rd Annual International Symposium on Computer Architecture (ISCA)},   title={Energy Efficient Architecture for Graph Analytics Accelerators},   year={2016},  volume={},  number={},  pages={166-177},  doi={10.1109/ISCA.2016.24}}

@inproceedings{dom5,
author = {Yan, Mingyu and Hu, Xing and Li, Shuangchen and Basak, Abanti and Li, Han and Ma, Xin and Akgun, Itir and Feng, Yujing and Gu, Peng and Deng, Lei and Ye, Xiaochun and Zhang, Zhimin and Fan, Dongrui and Xie, Yuan},
title = {Alleviating Irregularity in Graph Analytics Acceleration: A Hardware/Software Co-Design Approach},
year = {2019},
isbn = {9781450369381},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3352460.3358318},
doi = {10.1145/3352460.3358318},
abstract = {Graph analytics is an emerging application which extracts insights by processing large
volumes of highly connected data, namely graphs. The parallel processing of graphs
has been exploited at the algorithm level, which in turn incurs three irregularities
onto computing and memory patterns that significantly hinder an efficient architecture
design. Certain irregularities can be partially tackled by the prior domain-specific
accelerator designs with well-designed scheduling of data access, while others remain
unsolved.Unlike prior efforts, we fully alleviate these irregularities at their origin---the
data-dependent program behavior. To achieve this goal, we propose GraphDynS, a hardware/software
co-design with decoupled datapath and data-aware dynamic scheduling. Aware of data
dependencies extracted from the decoupled datapath, GraphDynS can elaborately schedule
the program on-the-fly to maximize parallelism. To extract data dependencies at runtime,
we propose a new programming model in synergy with a microarchitecture design that
supports datapath decoupling. Through data dependency information, we present several
data-aware strategies to dynamically schedule workloads, data accesses, and computations.
Overall, GraphDynS achieves 4.4\texttimes{} speedup and 11.6\texttimes{} less energy on average with half
the memory bandwidth compared to a state-of-the-art GPGPU-based solution. Compared
to a state-of-the-art graph analytics accelerator, GraphDynS also achieves 1.9\texttimes{} speedup
and 1.8\texttimes{} less energy on average using the same memory bandwidth.},
booktitle = {Proceedings of the 52nd Annual IEEE/ACM International Symposium on Microarchitecture},
pages = {615–628},
numpages = {14},
keywords = {graph analytics, accelerator, software and hardware co-design},
location = {Columbus, OH, USA},
series = {MICRO '52}
}

@inproceedings{micro-streaming1, author = {Basak, Abanti and Qu, Zheng and Lin, Jilan and Alameldeen, Alaa R. and Chishti, Zeshan and Ding, Yufei and Xie, Yuan}, title = {Improving Streaming Graph Processing Performance Using Input Knowledge}, year = {2021}, isbn = {9781450385572}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/3466752.3480096}, doi = {10.1145/3466752.3480096}, abstract = {Streaming graphs are ubiquitous in today’s big data era. Prior work has improved the performance of streaming graph workloads without taking input characteristics into account. In this work, we demonstrate that input knowledge-driven software and hardware co-design is critical to optimize the performance of streaming graph processing. To improve graph update efficiency, we first characterize the performance trade-offs of input-oblivious batch reordering. Guided by our findings, we propose input-aware batch reordering to adaptively reorder input batches based on their degree distributions. To complement adaptive batch reordering, we propose updating graphs dynamically, based on their input characteristics, either in software (via update search coalescing) or in hardware (via acceleration support). To improve graph computation efficiency, we present input-aware work aggregation which adaptively modulates the computation granularity based on inter-batch locality characteristics. Evaluated across 260 workloads, our input-aware techniques provide on average 4.55 \texttimes{} and 2.6 \texttimes{} improvement in graph update performance for different input types (on top of eliminating the performance degradation from input-oblivious batch reordering). The graph compute performance is improved by 1.26 \texttimes{} (up to 2.7 \texttimes{}). }, booktitle = {MICRO-54: 54th Annual IEEE/ACM International Symposium on Microarchitecture}, pages = {1036–1050}, numpages = {15}, keywords = {Graph analytics, Streaming graphs}, location = {Virtual Event, Greece}, series = {MICRO '21} }

@inproceedings{micro-streaming2, author = {Rahman, Shafiur and Afarin, Mahbod and Abu-Ghazaleh, Nael and Gupta, Rajiv}, title = {JetStream: Graph Analytics on Streaming Data with Event-Driven Hardware Accelerator}, year = {2021}, isbn = {9781450385572}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/3466752.3480126}, doi = {10.1145/3466752.3480126}, abstract = { Graph Processing is at the core of many critical emerging workloads operating on unstructured data, including social network analysis, bioinformatics, and many others. Many applications operate on graphs that are constantly changing, i.e., new nodes and edges are added or removed over time. In this paper, we present JetStream, a hardware accelerator for evaluating queries over streaming graphs and capable of handling additions, deletions, and updates of edges. JetStream extends a recently proposed event-based accelerator for graph workloads to support streaming updates. It handles both accumulative and monotonic graph algorithms via an event-driven computation model that limits accesses to a smaller subset of the graph vertices, efficiently reuses the prior query results to eliminate redundancy, and optimizes the memory access pattern for enhanced memory bandwidth utilization. To the best of our knowledge, JetStream is the first graph accelerator that supports streaming graphs, reducing the computation time by 90% compared with cold-start computation using an existing accelerator. In addition, JetStream achieves about 18 \texttimes{} speedup over KickStarter and GraphBolt software frameworks at the large baseline batch sizes that these systems use with significantly higher speedup at smaller batch sizes.}, booktitle = {MICRO-54: 54th Annual IEEE/ACM International Symposium on Microarchitecture}, pages = {1091–1105}, numpages = {15}, keywords = {incremental algorithms, accelerators, streaming graphs}, location = {Virtual Event, Greece}, series = {MICRO '21} }

@INPROCEEDINGS{graphpulse,
  author={Rahman, Shafiur and Abu-Ghazaleh, Nael and Gupta, Rajiv},
  booktitle={2020 53rd Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)}, 
  title={GraphPulse: An Event-Driven Hardware Accelerator for Asynchronous Graph Processing}, 
  year={2020},
  volume={},
  number={},
  pages={908-921},
  doi={10.1109/MICRO50266.2020.00078}}


@misc{snap,
  author       = {Jure Leskovec and Andrej Krevl},
  title        = {{SNAP Datasets}: {Stanford} Large Network Dataset Collection},
  howpublished = {\url{http://snap.stanford.edu/data}},
  month        = jun,
  year         = 2014
}

@INPROCEEDINGS{cacti,
    author = {Naveen Muralimanohar and others},
    title = {CACTI 6.0: A Tool to Understand Large Caches},
    booktitle={HP laboratories},
    year = {2009}
}


@article{ramulator, author = {Kim, Y. and Yang, W. and Mutlu, O.}, title = {Ramulator: A Fast and Extensible DRAM Simulator}, year = {2016}, issue_date = {January 2016}, publisher = {IEEE Computer Society}, address = {USA}, volume = {15}, number = {1}, issn = {1556-6056}, url = {https://doi.org/10.1109/LCA.2015.2414456}, doi = {10.1109/LCA.2015.2414456}, abstract = {Recently, both industry and academia have proposed many different roadmaps for the future of DRAM. Consequently, there is a growing need for an extensible DRAM simulator, which can be easily modified to judge the merits of today's DRAM standards as well as those of tomorrow. In this paper, we present Ramulator , a fast and cycle-accurate DRAM simulator that is built from the ground up for extensibility. Unlike existing simulators, Ramulator is based on a generalized template for modeling a DRAM system, which is only later infused with the specific details of a DRAM standard. Thanks to such a decoupled and modular design, Ramulator is able to provide out-of-the-box support for a wide array of DRAM standards: DDR3/4, LPDDR3/4, GDDR5, WIO1/2, HBM, as well as some academic proposals (SALP, AL-DRAM, TL-DRAM, RowClone, and SARP). Importantly, Ramulator does not sacrifice simulation speed to gain extensibility: according to our evaluations, Ramulator is 2.5 $times$ faster than the next fastest simulator. Ramulator is released under the permissive BSD license.}, journal = {IEEE Comput. Archit. Lett.}, month = jan, pages = {45–49}, numpages = {5} }

@article{pangolin,
author = {Chen, Xuhao and Dathathri, Roshan and Gill, Gurbinder and Pingali, Keshav},
title = {Pangolin: An Efficient and Flexible Graph Mining System on CPU and GPU},
year = {2020},
issue_date = {April 2020},
publisher = {VLDB Endowment},
volume = {13},
number = {8},
issn = {2150-8097},
url = {https://doi.org/10.14778/3389133.3389137},
doi = {10.14778/3389133.3389137},
abstract = {There is growing interest in graph pattern mining (GPM) problems such as motif counting.
GPM systems have been developed to provide unified interfaces for programming algorithms
for these problems and for running them on parallel systems. However, existing systems
may take hours to mine even simple patterns in moderate-sized graphs, which significantly
limits their real-world usability.We present Pangolin, an efficient and flexible in-memory
GPM framework targeting shared-memory CPUs and GPUs. Pangolin is the first GPM system
that provides high-level abstractions for GPU processing. It provides a simple programming
interface based on the extend-reduce-filter model, which allows users to specify application
specific knowledge for search space pruning and isomorphism test elimination. We describe
novel optimizations that exploit locality, reduce memory consumption, and mitigate
the overheads of dynamic memory allocation and synchronization.Evaluation on a 28-core
CPU demonstrates that Pangolin outperforms existing GPM frameworks Arabesque, RStream,
and Fractal by 49\texttimes{}, 88\texttimes{}, and 80\texttimes{} on average, respectively. Acceleration on a V100
GPU further improves performance of Pangolin by 15\texttimes{} on average. Compared to state-of-the-art
hand-optimized GPM applications, Pangolin provides competitive performance with less
programming effort.},
journal = {Proc. VLDB Endow.},
month = apr,
pages = {1190–1205},
numpages = {16}
}

@article{arabesque,
author = {Teixeira, Carlos H. C. and Fonseca, Alexandre J. and Serafini, Marco and Siganos, Georgos and Zaki, Mohammed J. and Aboulnaga, Ashraf},
title = {Arabesque: A System for Distributed Graph Mining},
year = {2015},
isbn = {9781450338349},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2815400.2815410},
abstract = {Distributed data processing platforms such as MapReduce and Pregel have substantially
simplified the design and deployment of certain classes of distributed graph analytics
algorithms. However, these platforms do not represent a good match for distributed
graph mining problems, as for example finding frequent subgraphs in a graph. Given
an input graph, these problems require exploring a very large number of subgraphs
and finding patterns that match some "interestingness" criteria desired by the user.
These algorithms are very important for areas such as social networks, semantic web,
and bioinformatics.In this paper, we present Arabesque, the first distributed data
processing platform for implementing graph mining algorithms. Arabesque automates
the process of exploring a very large number of subgraphs. It defines a high-level
filter-process computational model that simplifies the development of scalable graph
mining algorithms: Arabesque explores subgraphs and passes them to the application,
which must simply compute outputs and decide whether the subgraph should be further
extended. We use Arabesque's API to produce distributed solutions to three fundamental
graph mining problems: frequent subgraph mining, counting motifs, and finding cliques.
Our implementations require a handful of lines of code, scale to trillions of subgraphs,
and represent in some cases the first available distributed solutions.},
booktitle = {Proceedings of the 25th Symposium on Operating Systems Principles},
pages = {425–440},
numpages = {16}
}

@article{peregrine,
author = {Jamshidi, Kasra and Mahadasa, Rakesh and Vora, Keval},
title = {Peregrine: A Pattern-Aware Graph Mining System},
year = {2020},
isbn = {9781450368827},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3342195.3387548},
doi = {10.1145/3342195.3387548},
abstract = {Graph mining workloads aim to extract structural properties of a graph by exploring
its subgraph structures. General purpose graph mining systems provide a generic runtime
to explore subgraph structures of interest with the help of user-defined functions
that guide the overall exploration process. However, the state-of-the-art graph mining
systems remain largely oblivious to the shape (or pattern) of the subgraphs that they
mine. This causes them to: (a) explore unnecessary subgraphs; (b) perform expensive
computations on the explored subgraphs; and, (c) hold intermediate partial subgraphs
in memory; all of which affect their overall performance. Furthermore, their programming
models are often tied to their underlying exploration strategies, which makes it difficult
for domain users to express complex mining tasks.In this paper, we develop Peregrine,
a pattern-aware graph mining system that directly explores the subgraphs of interest
while avoiding exploration of unnecessary subgraphs, and simultaneously bypassing
expensive computations throughout the mining process. We design a pattern-based programming
model that treats graph patterns as first class constructs and enables Peregrine to
extract the semantics of patterns, which it uses to guide its exploration. Our evaluation
shows that Peregrine outperforms state-of-the-art distributed and single machine graph
mining systems, and scales to complex mining tasks on larger graphs, while retaining
simplicity and expressivity with its `pattern-first' programming approach.},
booktitle = {Proceedings of the Fifteenth European Conference on Computer Systems},
articleno = {13},
numpages = {16},
location = {Heraklion, Greece},
series = {EuroSys '20}
}

@article{rstream,
author = {Wang, Kai and Zuo, Zhiqiang and Thorpe, John and Nguyen, Tien Quang and Xu, Guoqing Harry},
title = {RStream: Marrying Relational Algebra with Streaming for Efficient Graph Mining on a Single Machine},
year = {2018},
isbn = {9781931971478},
publisher = {USENIX Association},
address = {USA},
abstract = {Graph mining is an important category of graph algorithms that aim to discover structural
patterns such as cliques and motifs in a graph. While a great deal of work has been
done recently on graph computation such as PageRank, systems support for scalable
graph mining is still limited. Existing mining systems such as Arabesque focus on
distributed computing and need large amounts of compute and memory resources.We built
RStream, the first single-machine, out-of-core mining system that leverages disk support
to store intermediate data. At its core are two innovations: (1) a rich programming
model that exposes relational algebra for developers to express a wide variety of
mining tasks; and (2) a runtime engine that implements relational algebra efficiently
with tuple streaming. A comparison between RStream and four state-of-the-art distributed
mining/Datalog systems--Arabesque, ScaleMine, DistGraph, and BigDatalog -- demonstrates
that RStream outperforms all of them, running on a 10-node cluster, e.g., by at least
a factor of 1.7\texttimes{}, and can process large graphs on an inexpensive machine.},
booktitle = {Proceedings of the 13th USENIX Conference on Operating Systems Design and Implementation},
pages = {763–782},
numpages = {20},
location = {Carlsbad, CA, USA},
series = {OSDI'18}
}

@article{peregrine_followup, author = {Jamshidi, Kasra and Vora, Keval}, title = {A Deeper Dive into Pattern-Aware Subgraph Exploration with PEREGRINE}, year = {2021}, issue_date = {July 2021}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, volume = {55}, number = {1}, issn = {0163-5980}, url = {https://doi.org/10.1145/3469379.3469381}, doi = {10.1145/3469379.3469381}, abstract = {Graph mining workloads aim to extract structural properties of a graph by exploring its subgraph structures. PEREGRINE is a general-purpose graph mining system that provides a generic runtime to efficiently explore subgraph structures of interest and perform various graph mining analyses. It takes a 'pattern-aware' approach by incorporating a pattern-based programming model along with efficient pattern matching strategies. The programming model enables easier expression of complex graph mining use cases and enables PEREGRINE to extract the semantics of patterns. By analyzing the patterns, PEREGRINE generates efficient exploration plans which it uses to guide its subgraph exploration.In this paper, we present an in-depth view of the patternanalysis techniques powering the matching engine of PEREGRINE. Beyond the theoretical foundations from prior research, we expose opportunities based on how the exploration plans are evaluated, and develop key techniques for computation reuse, enumeration depth reduction, and branch elimination. Our experiments show the importance of patternawareness for scalable and performant graph mining where the presented new techniques speed up the performance by up to two orders of magnitude on top of the benefits achieved from the prior theoretical foundations that generate the initial exploration plans.}, journal = {SIGOPS Oper. Syst. Rev.}, month = jun, pages = {1–10}, numpages = {10} }

@inproceedings{graphzero,
  title={Graphzero: Breaking symmetry for efficient graph mining},
  author={D. Mawhirter and S. Reinehr and C. Holmes and T. Liu and and B. Wu},
  booktitle={arXiv preprint arXiv:1911.12877},
  year={2019}
}

@article{automine,
author = {Mawhirter, Daniel and Wu, Bo},
title = {AutoMine: Harmonizing High-Level Abstraction and High Performance for Graph Mining},
year = {2019},
isbn = {9781450368735},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3341301.3359633},
doi = {10.1145/3341301.3359633},
abstract = {Graph mining algorithms that aim at identifying structural patterns of graphs are
typically more complex than graph computation algorithms such as breadth first search.
Researchers have implemented several systems with high-level and flexible interfaces
customized for tackling graph mining problems. However, we find that for triangle
counting, one of the simplest graph mining problems, such systems can be several times
slower than a single-threaded implementation of a straightforward algorithm.In this
paper, we reveal the root causes of the severe inefficiencies of state-of-the-art
graph mining systems and the challenges to address the performance problems. We build
AutoMine, a single-machine system to provide both high-level interfaces and high performance
for large-scale graph mining applications. The novelty of AutoMine comes from 1) a
new representation of subgraph patterns and 2) compilation techniques that automatically
generate efficient mining code with minimized memory consumption from a high-level
abstraction. We have extensively evaluated AutoMine against 3 graph mining systems
on 8 real-world graphs of different scales. Our experimental results show that AutoMine
often produces several orders of magnitude better performance and can process very
large graphs existing systems cannot handle.},
booktitle = {Proceedings of the 27th ACM Symposium on Operating Systems Principles},
pages = {509–523},
numpages = {15},
keywords = {compiler, graph pattern matching, graph mining},
location = {Huntsville, Ontario, Canada},
series = {SOSP '19}
}


@article{fractal,
author = {Dias, Vinicius and Teixeira, Carlos H. C. and Guedes, Dorgival and Meira, Wagner and Parthasarathy, Srinivasan},
title = {Fractal: A General-Purpose Graph Pattern Mining System},
year = {2019},
isbn = {9781450356435},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3299869.3319875},
doi = {10.1145/3299869.3319875},
abstract = {In this paper we propose Fractal, a high performance and high productivity system
for supporting distributed graph pattern mining (GPM) applications. Fractal employs
a dynamic (auto-tuned) load-balancing based on a hierarchical and locality-aware work
stealing mechanism, allowing the system to adapt to different workload characteristics.
Additionally, Fractal enumerates subgraphs by combining a depth-first strategy with
a from scratch processing paradigm to avoid storing large amounts of intermediate
state and, thus, improves memory efficiency. Regarding programmer productivity, Fractal
presents an intuitive, expressive and modular API, allowing for rapid compositional
expression of many GPM algorithms. Fractal-based implementations outperform both existing
systemic solutions and specialized distributed solutions on many problems - from frequent
graph mining to subgraph querying, over a range of datasets.},
booktitle = {Proceedings of the 2019 International Conference on Management of Data},
pages = {1357–1374},
numpages = {18},
keywords = {graph pattern mining, distributed systems},
location = {Amsterdam, Netherlands},
series = {SIGMOD '19}
}

@inproceedings{ainsworth_graph,
 author = {Ainsworth, S. and Jones, T. M.},
 title = {Graph Prefetching Using Data Structure Knowledge},
 booktitle = {ICS},
 year = {2016},
 isbn = {978-1-4503-4361-9},
 location = {Istanbul, Turkey},
 pages = {39:1--39:11},
 articleno = {39},
 numpages = {11},
 doi = {10.1145/2925426.2926254},
 acmid = {2926254},
 address = {New York, NY, USA},
 keywords = {Graphs, Prefetching},
} 

@INPROCEEDINGS{droplet, 
author={Basak, Abanti and Li, Shuangchen and Hu, Xing and Oh, Sang Min and Xie, Xinfeng and Zhao, Li and Jiang, Xiaowei and Xie, Yuan}, 
booktitle={HPCA}, 
title={Analysis and Optimization of the Memory Hierarchy for Graph Processing Workloads}, 
year={2019}, 
volume={}, 
number={}, 
pages={373-386}, 
keywords={Big Data;cache storage;graph theory;multiprocessing systems;parallel processing;storage management;in-memory graph analytics;memory hierarchy;cache hierarchy;load-load dependency chains;DROPLET;big data applications;graph processing;memory-level parallelism;application data types;graph data types;data-aware decoupled prefetcher;private L2 cache;shared L3 cache;Prefetching;Random access memory;Arrays;Parallel processing;Hardware;Benchmark testing;Graph Processing;Workload Characterization;Prefetching}, 
doi={10.1109/HPCA.2019.00051}, 
ISSN={2378-203X}, 
month={Feb},}

@inproceedings{dom6,
  title={Cache-Guided Scheduling : Exploiting Caches to Maximize Locality in Graph Processing},
  author={Nathan Beckmann and Daniel S{\'a}nchez},
  year={2017}
}

@INPROCEEDINGS{dom2,  author={Singapura, Shreyas G. and Srivastava, Ajitesh and Kannan, Rajgopal and Prasanna, Viktor K.},  booktitle={2017 IEEE High Performance Extreme Computing Conference (HPEC)},   title={OSCAR: Optimizing SCrAtchpad reuse for graph processing},   year={2017},  volume={},  number={},  pages={1-7},  doi={10.1109/HPEC.2017.8091070}}

@article{prodigy,  author={Talati, Nishil and May, Kyle and Behroozi, Armand and Yang, Yichen and Kaszyk, Kuba and Vasiladiotis, Christos and Verma, Tarunesh and Li, Lu and Nguyen, Brandon and Sun, Jiawen and Morton, John Magnus and Ahmadi, Agreen and Austin, Todd and O’Boyle, Michael and Mahlke, Scott and Mudge, Trevor and Dreslinski, Ronald},  booktitle={2021 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},   title={Prodigy: Improving the Memory Latency of Data-Indirect Irregular Workloads Using Hardware-Software Co-Design},   year={2021},  volume={},  number={},  pages={654-667},  doi={10.1109/HPCA51647.2021.00061}}

@inproceedings{segura2019scu,
  title={SCU: a GPU stream compaction unit for graph processing},
  author={Segura, Albert and Arnau, Jose-Maria and Gonz{\'a}lez, Antonio},
  booktitle={2019 ACM/IEEE 46th Annual International Symposium on Computer Architecture (ISCA)},
  pages={424--435},
  year={2019},
  organization={IEEE}
}

@inproceedings{mukkara:micro:2019:phi,
 author = {Anurag Mukkara and Nathan Beckmann and Daniel Sanchez},
 title = {{PHI: Architectural Support for Synchronization-and Bandwidth-Efficient Commutative Scatter Updates}},
 booktitle = {Proceedings of the 52nd annual IEEE/ACM international symposium on Microarchitecture (MICRO-52)},
 month = {October},
 year = {2019},
}

@inproceedings{triejax,
author = {Kalinsky, Oren and Kimelfeld, Benny and Etsion, Yoav},
title = {The TrieJax Architecture: Accelerating Graph Operations Through Relational Joins},
year = {2020},
isbn = {9781450371025},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3373376.3378524},
doi = {10.1145/3373376.3378524},
abstract = {Graph pattern matching (e.g., finding all cycles and cliques) has become an important
component in domains such as social networks, biology and cyber-security. In recent
years, the database community has shown that graph pattern matching problems can be
mapped to an efficient new class of relational join algorithms.In this paper, we argue
that this new class of join algorithms is highly amenable to specialized hardware
acceleration thanks to two fundamental properties: improved memory locality and inherent
concurrency. The improved locality is a result of the bound number of intermediate
results these algorithms generate, which yields smaller working sets. Coupled with
custom caching mechanisms, this property can be used to dramatically reduce the number
of main memory accesses invoked by the algorithm. In addition, their inherent concurrency
can be leveraged for effective hardware acceleration and hiding memory latency.We
demonstrate the hardware amenability of this new class of algorithms by introducing
TrieJax, a hardware accelerator for graph pattern matching that can be tightly integrated
into existing manycore processors. TrieJax employs custom caching mechanisms and a
massively multithreaded design to dramatically accelerate graph pattern matching.
We evaluate TrieJax on a set standard graph pattern matching queries and datasets.
Our evaluation shows that TrieJax outperforms recently proposed hardware accelerators
for graph and database processing that do not employ the new class of algorithms by
7 - 63\texttimes{} on average (up to 539\texttimes{}), while consuming 15 - 179\texttimes{} less energy (up to 1750\texttimes{}),
and systems that incorporate modern relational join algorithms by 9 - 20\texttimes{} on average
(up to 45\texttimes{}), while consuming 59 - 110\texttimes{} less energy (up to 372\texttimes{}).},
booktitle = {Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
pages = {1217–1231},
numpages = {15},
keywords = {relational join, hardware and algorithmic design, hardware acceleration, graph analytics, databases},
location = {Lausanne, Switzerland},
series = {ASPLOS '20}
}

@article{sisa,
  title={SISA: Set-Centric Instruction Set Architecture for Graph Mining on Processing-in-Memory Systems}, 
  author={Maciej Besta and Raghavendra Kanakagiri and Grzegorz Kwasniewski and Rachata Ausavarungnirun and Jakub Beránek and Konstantinos Kanellopoulos and Kacper Janda and Zur Vonarburg-Shmaria and Lukas Gianinazzi and Ioana Stefan and Juan Gómez Luna and Marcin Copik and Lukas Kapp-Schwoerer and Salvatore Di Girolamo and Marek Konieczny and Onur Mutlu and Torsten Hoefler},
  year={2021},
  journal={2021 54th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)}
}

@inproceedings{cpi-stack-methodology, author = {Eyerman, Stijn and Eeckhout, Lieven and Karkhanis, Tejas and Smith, James E.}, title = {A Performance Counter Architecture for Computing Accurate CPI Components}, year = {2006}, isbn = {1595934510}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/1168857.1168880}, doi = {10.1145/1168857.1168880}, abstract = {A common way of representing processor performance is to use Cycles per Instruction (CPI) `stacks' which break performance into a baseline CPI plus a number of individual miss event CPI components. CPI stacks can be very helpful in gaining insight into the behavior of an application on a given microprocessor; consequently, they are widely used by software application developers and computer architects. However, computing CPI stacks on superscalar out-of-order processors is challenging because of various overlaps among execution and miss events (cache misses, TLB misses, and branch mispredictions).This paper shows that meaningful and accurate CPI stacks can be computed for superscalar out-of-order processors. Using interval analysis, a novel method for analyzing out-of-order processor performance, we gain understanding into the performance impact of the various miss events. Based on this understanding, we propose a novel way of architecting hardware performance counters for building accurate CPI stacks. The additional hardware for implementing these counters is limited and comparable to existing hardware performance counter architectures while being significantly more accurate than previous approaches.}, booktitle = {Proceedings of the 12th International Conference on Architectural Support for Programming Languages and Operating Systems}, pages = {175–184}, numpages = {10}, keywords = {hardware performance counter architecture, superscalar processor performance modeling}, location = {San Jose, California, USA}, series = {ASPLOS XII} }

@inproceedings{iyer2018asap,
  title={$\{$ASAP$\}$: Fast, approximate graph pattern mining at scale},
  author={Iyer, Anand Padmanabha and Liu, Zaoxing and Jin, Xin and Venkataraman, Shivaram and Braverman, Vladimir and Stoica, Ion},
  booktitle={13th USENIX Symposium on Operating Systems Design and Implementation (OSDI 18)},
  pages={745--761},
  year={2018}
}

@inproceedings{reza2020approximate,
  title={Approximate pattern matching in massive graphs with precision and recall guarantees},
  author={Reza, Tashin and Ripeanu, Matei and Sanders, Geoffrey and Pearce, Roger},
  booktitle={Proceedings of the 2020 ACM SIGMOD International Conference on Management of Data},
  pages={1115--1131},
  year={2020}
}

@inproceedings{preti2021maniacs,
  title={MaNIACS: Approximate Mining of Frequent Subgraph Patterns through Sampling},
  author={Preti, Giulia and De Francisci Morales, Gianmarco and Riondato, Matteo},
  booktitle={Proceedings of the 27th ACM SIGKDD Conference on Knowledge Discovery \& Data Mining},
  pages={1348--1358},
  year={2021}
}

@inproceedings{dai2022dimmining,
  title={DIMMining: pruning-efficient and parallel graph mining on near-memory-computing},
  author={Dai, Guohao and Zhu, Zhenhua and Fu, Tianyu and Wei, Chiyue and Wang, Bangyan and Li, Xiangyu and Xie, Yuan and Yang, Huazhong and Wang, Yu},
  booktitle={Proceedings of the 49th Annual International Symposium on Computer Architecture},
  pages={130--145},
  year={2022}
}

@inproceedings{chronos,
  title={Chronos: Efficient speculative parallelism for accelerators},
  author={Abeydeera, Maleen and Sanchez, Daniel},
  booktitle={Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={1247--1262},
  year={2020}
}

@inproceedings{matraptor,
  title={Matraptor: A sparse-sparse matrix multiplication accelerator based on row-wise product},
  author={Srivastava, Nitish and Jin, Hanchen and Liu, Jie and Albonesi, David and Zhang, Zhiru},
  booktitle={2020 53rd Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={766--780},
  year={2020},
  organization={IEEE}
}

@inproceedings{zhang2020sparch,
  title={Sparch: Efficient architecture for sparse matrix multiplication},
  author={Zhang, Zhekai and Wang, Hanrui and Han, Song and Dally, William J},
  booktitle={2020 IEEE International Symposium on High Performance Computer Architecture (HPCA)},
  pages={261--274},
  year={2020},
  organization={IEEE}
}

@inproceedings{pal2018outerspace,
  title={Outerspace: An outer product based sparse matrix multiplication accelerator},
  author={Pal, Subhankar and Beaumont, Jonathan and Park, Dong-Hyeon and Amarnath, Aporva and Feng, Siying and Chakrabarti, Chaitali and Kim, Hun-Seok and Blaauw, David and Mudge, Trevor and Dreslinski, Ronald},
  booktitle={2018 IEEE International Symposium on High Performance Computer Architecture (HPCA)},
  pages={724--736},
  year={2018},
  organization={IEEE}
}

@article{lin2013design,
  title={Design space exploration for sparse matrix-matrix multiplication on FPGAs},
  author={Lin, Colin Yu and Wong, Ngai and So, Hayden Kwok-Hay},
  journal={International Journal of Circuit Theory and Applications},
  volume={41},
  number={2},
  pages={205--219},
  year={2013},
  publisher={Wiley Online Library}
}

@article{han2016eie,
  title={EIE: Efficient inference engine on compressed deep neural network},
  author={Han, Song and Liu, Xingyu and Mao, Huizi and Pu, Jing and Pedram, Ardavan and Horowitz, Mark A and Dally, William J},
  journal={ACM SIGARCH Computer Architecture News},
  volume={44},
  number={3},
  pages={243--254},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@article{zachariadis2020accelerating,
  title={Accelerating sparse matrix--matrix multiplication with GPU Tensor Cores},
  author={Zachariadis, Orestis and Satpute, Nitin and G{\'o}mez-Luna, Juan and Olivares, Joaqu{\'\i}n},
  journal={Computers \& Electrical Engineering},
  volume={88},
  pages={106848},
  year={2020},
  publisher={Elsevier}
}

@misc{yamaguchi2021accelerating,
  title={Accelerating Matrix Multiplication with Block Sparse Format and NVIDIA Tensor Cores},
  author={Yamaguchi, Takuma and Busato, Federico},
  year={2021}
}
www
@inproceedings{jouppi2017datacenter,
  title={In-datacenter performance analysis of a tensor processing unit},
  author={Jouppi, Norman P. and Young, Cliff and Patil, Nishant and Patterson, David and Agrawal, Gaurav and Bajwa, Raminder and Bates, Sarah and Bhatia, Suresh and Boden, Nan and Borchers, Al and Boyle, Rick and Cantin, Pierre-luc and Chao, Clifford and Clark, Chris and Coriell, Jeremy and Daley, Mike and Dau, Matt and Dean, Jeffrey and Gelb, Ben and Ghaemmaghami, Tara Vazir and Gottipati, Rajendra and Gulland, William and Hagmann, Robert and Ho, C. Richard and Hogberg, Doug and Hu, John and Hundt, Robert and Hurt, Dan and Ibarz, Julian and Jaffey, Aaron and Jaworski, Alek and Kaplan, Alexander and Khaitan, Harshit and Killebrew, Daniel and Koch, Andy and Kumar, Naveen and Lacy, Steve and Laudon, James and Law, James and Le, Diemthu and Leary, Chris and Liu, Zhuyuan and Lucke, Kyle and Lundin, Alan and MacKean, Gordon and Maggiore, Adriana and Mahony, Maire and Miller, Kieran and Nagarajan, Rahul and Narayanaswami, Ravi and Ni, Ray and Nix, Kathy and Norrie, Thomas and Omernick, Mark and Penukonda, Narayana and Phelps, Andy and Ross, Jonathan and Ross, Matt and Salek, Amir and Samadiani, Emad and Severn, Chris and Sizikov, Gregory and Snelham, Matthew and Souter, Jed and Steinberg, Dan and Swing, Andy and Tan, Mercedes and Thorson, Gregory and Tian, Bo and Toma, Horia and Tuttle, Erick and Vasudevan, Vijay and Walter, Richard and Wang, Walter and Wilcox, Eric and Yoon, Doe Hyun},
  booktitle={Proceedings of the 44th annual international symposium on computer architecture},
  pages={1--12},
  year={2017}
}

@misc{snap_opensource,
    author = {Paranjape, Ashwin and Benson, Austin R and Leskovec, Jure},
    title = {{Temporal motifs code in SNAP}},
    url = "https://snap.stanford.edu/temporal-motifs/code.html",
  }
